On Using GUI Interaction Data to Improve Text Retrieval-based Bug Localization

One of the most important tasks related to managing bug reports is localizing the fault so that a fix can be applied. As such, prior work has aimed to automate this task of bug localization by formulating it as an information retrieval problem, where potentially buggy files are retrieved and ranked according to their textual similarity with a given bug report. However, there is often a notable semantic gap between the information contained in bug reports and identifiers or natural language contained within source code files. For user-facing software, there is currently a key source of information that could aid in bug localization, but has not been thoroughly investigated - information from the GUI. We investigate the hypothesis that, for end user-facing applications, connecting information in a bug report with information from the GUI, and using this to aid in retrieving potentially buggy files, can improve upon existing techniques for bug localization. To examine this phenomenon, we conduct a comprehensive empirical study that augments four baseline techniques for bug localization with GUI interaction information from a reproduction scenario to (i) filter out potentially irrelevant files, (ii) boost potentially relevant files, and (iii) reformulate text-retrieval queries. To carry out our study, we source the current largest dataset of fully-localized and reproducible real bugs for Android apps, with corresponding bug reports, consisting of 80 bug reports from 39 popular open-source apps. Our results illustrate that augmenting traditional techniques with GUI information leads to a marked increase in effectiveness across multiple metrics, including a relative increase in Hits@10 of 13-18%. Additionally, through further analysis, we find that our studied augmentations largely complement existing techniques.

==> discussion.tex <==
\section{Discussion and Learned Lessons}
\subsection{Lesson 1: Generate crowd-sourced usage data for diverse configurations of emulators.}
For the AndroR2 \cite{Wendland2021, Johnson2022} dataset, the authors used the specific Android versions mentioned in the bug reports in order to reproduce the bugs. The reproduction scripts are written in a specific way that bugs should be reproduced on specific emulator settings. This requirement is expected since all bugs cannot be reproduced in all emulator versions. Furthermore, many bugs require specific settings that cannot be found in other emulators.

However, our trace-replayer data is collected in a way that bugs need to be reproduced only on \texttt{Nexus 5X API 24}. Therefore, we first checked whether the bugs could be reproduced on this emulator and generated trace-replayer data. However, not all bugs can be reproduced on this specific emulator. Therefore, currently, we work with the data where we are able to reproduce bugs on this specific emulator. We aim to update the process for the generation of the trace-replayer data so that we can work with more bugs that are reproducible in different configurations of the emulator.

\subsection{Lesson 2: We cannot perform source code mapping only based on the final application state.}
Our main goal is to identify the last application state before the bug occurs and use that information to locate the buggy source code. Unfortunately, we are not able to map the state to the source code based on the final application state in all cases. More specifically, out of the six analyzed bug reports, the bug occurs after clicking on the BACK button on the navigation bar in two cases. There is no target GUI component in the last graph transition in this scenario. Consequently, we do not have enough information to locate the buggy files only based on the last transition and need to use the past few transitions in the graph for bug localization. For instance, in one of the cases, the bug occurs after the user starts the voice recording and clicks on the BACK button. In this case, we use the graph transition right before the final transition to obtain the actual GUI component data.

We aim to perform a motivational study to understand which application states are necessary to map the bug report to the source code. Moreover, we want to investigate what percentage of the bugs can be localized by only leveraging the final application state.

\subsection{Lesson 3: Our graph-based approach can identify any type of buggy source code file, however, approaches like BugLocator cannot identify buggy XML files.}

Most of the previous bug localization techniques used open-source projects to locate buggy files. Many previous approaches aimed to locate Java files, while our approach is designed for mobile apps that include XML files. Some of the bugs are only related to XML files without locating any Java or other types of files. Previous approaches like BugLocator \cite{Zhou2012}, which is used as one of our baselines, are specifically designed for locating Java files. When we leveraged that approach for our dataset, we could not locate XML files. This limitation makes such approaches unable to localize specific bugs like GUI issues in Android applications. However, our graph-based approach can locate any source code file, including XML files in Android projects. 

\subsection{Lesson 4: We need to perform a motivational study to improve our source code mapping technique.}
So far, we have analyzed six bug reports and Android applications to design our source code mapping technique. We believe that by analyzing more bug reports and Android applications, we should come up with more effective heuristics for bug localization. For instance, we might find out that specific XML attributes related to the target GUI component could more accurately lead us to the pieces of code where that component is used.
